The Variation of Magnesium Depletion with Line of Sight Conditions

In this paper we report on the gas-phase abundance of singly-ionized magnesium (Mg II) in 44 lines of sight, using data from the Hubble Space Telescope (HST). We measure Mg II column densities by analyzing medium- and high-resolution archival STIS spectra of the 1240 A doublet of Mg II. We find that Mg II depletion is correlated with many line of sight parameters (e.g. F(H_2), E_(B-V), E_(B-V)/r, A_V, and A_V/r) in addition to the well-known correlation with <n_H>. These parameters should be more directly related to dust content and thus have more physical significance with regard to the depletion of elements such as magnesium. We examine the significance of these additional correlations as compared to the known correlation between Mg II depletion and <n_H>. While none of the correlations are better predictors of Mg II depletion than <n_H>, some are statistically significant even assuming fixed <n_H>. We discuss the ranges over which these correlations are valid, their strength at fixed <n_H>, and physical interpretations.

==> macros.tex <==
\newtheorem{theorem}{Theorem}


\newcommand{\diff}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\diffr}[1]{\diff{#1}{r}}
\newcommand{\diffth}[1]{\diff{#1}{\theta}}
\newcommand{\diffz}[1]{\diff{#1}{z}}

\newcommand{\vth}{V_{\theta}}

\newcommand{\twochoices}[2]{\left\{ \begin{array}{lcc}
        \displaystyle #1 \\ \vspace{-10pt} \\
        \displaystyle #2 \end{array} \right. } %}

\newcommand{\threechoices}[3]{\left\{ \begin{array}{lcc}
        #1 \\ #2 \\ #3 \end{array} \right. }    %}

\newcommand{\fourchoices}[4]{\left\{ \begin{array}{lcc}
        #1 \\ #2 \\ #3 \\ #4 \end{array} \right. }      %}

\newcommand{\twovec}[2]{\left(\begin{array}{c} #1 \\ #2 \end{array}\right)}
\newcommand{\threevec}[3]{\left(\begin{array}{c} #1 \\ #2 \\ #3 \end{array}\right)}
\newcommand{\twomatrix}[4]{\left(\begin{array}{cc} #1 & #2 \\ #3 & #4 \end{array}\right)}

% Solar commands
\newcommand{\mdot}{{\dot{\rm M}}}
\newcommand{\msun}{{~{\rm M}_\odot}}
\newcommand{\msunperyr}{{\msun {\rm yr}^{-1}}}
% Unit commands
\newcommand{\kmpers}{{{\rm \; km\;s}^{-1}}}
\newcommand{\ppm}{{\rm \; ppm}}
\newcommand{\percc}{{\rm \; cm}^{-3}}
\newcommand{\dex}{{\rm \; dex}}
\newcommand{\magnitude}{{\rm \; mag}}
% Abundance commands
\newcommand{\logOH}{{\log{{\rm(O/H)}}}}
\newcommand{\logNH}{{\log{{\rm(N/H)}}}}
\newcommand{\logFeH}{{\log{{\rm(Fe/H)}}}}
\newcommand{\logFeIIH}{{\log{{\rm(Fe \; II/H)}}}}
\newcommand{\logMgH}{{\log{{\rm(Mg/H)}}}}
\newcommand{\logMgIIH}{{\log{{\rm(Mg \; II/H)}}}}
\newcommand{\logSiH}{{\log{{\rm(Si/H)}}}}
\newcommand{\logSiIIH}{{\log{{\rm(Si \; II/H)}}}}
\newcommand{\Htot}{{\rm H_{tot}}}
\newcommand{\OH}{{\rm O/H}}
\newcommand{\NH}{{\rm N/H}}
\newcommand{\FeH}{{\rm Fe/H}}
\newcommand{\MgH}{{\rm Mg/H}}
\newcommand{\SiH}{{\rm Si/H}}
\newcommand{\OHsolar}{{\rm(O/H)}_{\odot}}
\newcommand{\OHdust}{{\rm O_{dust}/H}}
%Column density commands
\newcommand{\NHI}{{N{\rm(H \; I)}}}
\newcommand{\NOI}{{N{\rm(O \; I)}}}
\newcommand{\NNI}{{N{\rm(N \; I)}}}
\newcommand{\NHmol}{{N\rm(H_{2})}}
\newcommand{\NFe}{{N{\rm(Fe)}}}
\newcommand{\NFeII}{{N{\rm(Fe \; II)}}}
\newcommand{\logFeII}{{\log{N{\rm(Fe \; II)}}}}
\newcommand{\NMg}{{N{\rm(Mg)}}}
\newcommand{\NMgII}{{N{\rm(Mg \; II)}}}
\newcommand{\logMgII}{{\log{N{\rm(Mg \; II)}}}}
\newcommand{\NSi}{{N{\rm(Mg)}}}
\newcommand{\NSiII}{{N{\rm(Si \; II)}}}
\newcommand{\logSiII}{{\log{N{\rm(Si \; II)}}}}
\newcommand{\logHI}{{\log{\NHI}}}
\newcommand{\logHmol}{{\log{\NHmol}}}
\newcommand{\logHtot}{{\log{\NHtot}}}
\newcommand{\logOI}{{\log{N\rm(O \; I)}}}
\newcommand{\logNI}{{\log{N\rm(N \; I)}}}
\newcommand{\NHtot}{{N{\rm(H_{tot})}}}
% Molecular commands
\newcommand{\Hmol}{{\rm H_{2}}}
\newcommand{\Nmol}{{\rm N_{2}}}
% Line of sight parameter commands
\newcommand{\nH}{{\rm{n_{H}}}}
%\newcommand{\nHavg}{{\langle \rm{n_{H}} \rangle}}
\newcommand{\nHavg}{{< \! \! \rm{n_{H}} \! \! >}}
\newcommand{\nHvol}{{\rm n_{H}}}
\newcommand{\lognh}{{\log{\nH}}}
\newcommand{\lognHavg}{{\log{\nHavg}}}
\newcommand{\lognha}{{\log{\nHavg}}}
\newcommand{\fHmol}{{f\rm(H_{2})}}
% Other commands
\newcommand{\eqw}{{W_{\lambda}}}
\newcommand{\av}{{A_V}}
\newcommand{\alamb}{{A_{\lambda}}}
\newcommand{\ebv}{{E_{B-V}}}
\newcommand{\elambv}{{E_{\lambda-V}}}
\newcommand{\avdist}{{\av / r}}
\newcommand{\ebvdist}{{\ebv / r}}
\newcommand{\rv}{{R_V}}
\newcommand{\nelec}{{\rm n_{e}}}
